HyperService: Interoperability and Programmability Across Heterogeneous Blockchains

Blockchain interoperability, which allows state transitions across different blockchain networks, is critical functionality to facilitate major blockchain adoption. Existing interoperability protocols mostly focus on atomic token exchange between blockchains. However, as blockchains have been upgraded from passive distributed ledgers into programmable state machines (thanks to smart contracts), the scope of blockchain interoperability goes beyond just token exchange. In this paper, we present HyperService, the first platform that delivers interoperability and programmability across heterogeneous blockchains. HyperService is powered by two innovative designs: (i) a developer-facing programming framework that allows developers to build cross-chain applications in a unified programming model; and (ii) a secure blockchain-facing cryptography protocol that provably realizes those applications on blockchains. We implement a prototype of HyperService in about 35,000 lines of code to demonstrate its practicality. Our experiment results show that HyperService imposes reasonable latency, in order of seconds, on the end-to-end execution of cross-chain applications

==> ven_arch.tex <==
\subsection{Architecture of \VENs}\label{sec:ven_arch}
In this section, we discuss the architecture of \VENs, including 
\VEN discovery and the anatomy of a \VEN. 
In order to find a \VEN, a \dApp relies on 
a \emph{directory} (similar to the Tor's relay directories~\cite{tor,tor-da}),
which we envision to be an informal list of \VENs
together with their operation models. 
Developers chooses a \VEN that matches their 
\dApp requirements, including sufficient blockchain reachability by the \VEN, reasonable 
service fee, and sufficient trustworthiness for execution. 
For example, a \dApp may prefer a \VEN with 
Intel SGX~\cite{costan16intel} capability 
for privacy-preserving computation~\cite{m2r,opaque,vc3}. 
Since all \dApp execution results are 
publicly verifiable, it is possible to build a \VEN reputation 
system to provide a valuable metric for \VEN selection. 
The \VEN thus misbehaves at its own risk. 
% Some \VENs may limit the amount they stake for a single \Op
% to bound losses in case of \VEN failures.

A \VEN itself is a distributed system,  
executing transactions across potentially several
\emph{isolation domains}.
For example, the \VEN may execute lower-value 
transactions together, perhaps even on cloud infrastructure,
but execute higher-value transactions on dedicated machines,
limiting the risk of key exfiltration from
operating system or even hardware vulnerabilities
such as Meltdown, Spectre,
and RowHammer~\cite{meltdown, spectre, row-hammer}.
If an isolation domain fails, the \VEN's risk is limited
to \Ops that are currently executing in that domain.
Within an isolation domain, a \VEN may further 
operate several machines 
to limit the number of BNs in which each machine
needs to participate as a fullnode, as well as 
balancing the mapping between 
transaction intents and nodes. 

Furthermore, in order to improve availability,
a \VEN may designate one or more backup nodes
for each transaction intent.
To ensure that each transaction is executed exactly once,
the \VEN must ensure that no matter which node generates the transaction,
the transaction is bitwise identical. Towards this end, 
the \VEN uses a common pool of randomness
to generate random numbers (\eg keys) for that transaction.
For example, the \VEN may assign each \Op a secret randomness key $k$.
Then for generating the $i$-th transaction,
\VEN nodes use $\mbox{PRF}_k(i)$ as a randomness seed;
within the a transaction, to generate the $j$-th random number for transaction $i$,
\VEN nodes use the value $\mbox{PRF}_{\mbox{PRF}_k(i)}(j)$.

Due to limitations in the size of funds 
that a \VEN may wish to stake to the \ISC,
a \dApp may be too large for any single \VEN.
Alternatively, a \dApp may span a set of BNs
such that no single \VEN has the reachability to 
all of them. In such cases, a \dApp could be 
executed by a collection of \VENs. In general, 
\sys is not limited by such multi-\VEN execution 
as long as the \ISC is instantiated properly with correct 
reversion accounts and finer-grained arbitration logic. 


